Optimal Multi-Unit Mechanisms with Private Demands

In the multi-unit pricing problem, multiple units of a single item are for sale. A buyer's valuation for $n$ units of the item is $v \min \{ n, d\} $, where the per unit valuation $v$ and the capacity $d$ are private information of the buyer. We consider this problem in the Bayesian setting, where the pair $(v,d)$ is drawn jointly from a given probability distribution. In the \emph{unlimited supply} setting, the optimal (revenue maximizing) mechanism is a pricing problem, i.e., it is a menu of lotteries. In this paper we show that under a natural regularity condition on the probability distributions, which we call \emph{decreasing marginal revenue}, the optimal pricing is in fact \emph{deterministic}. It is a price curve, offering $i$ units of the item for a price of $p_i$, for every integer $i$. Further, we show that the revenue as a function of the prices $p_i$ is a \emph{concave} function, which implies that the optimum price curve can be found in polynomial time. This gives a rare example of a natural multi-parameter setting where we can show such a clean characterization of the optimal mechanism. We also give a more detailed characterization of the optimal prices for the case where there are only two possible demands.

==> characterizations.tex <==
\section{Characterizations}

Our objective is to maximize revenue, i.e. $\sum_{d_i = 1}^D \int_0^{\bar{V}} \p{v,d_i} f(v,d_i) dv$. Using the payment formula for a fixed $d$, changing the order of inegration and using integration by parts \`a la Myerson, we can rewrite this objective as:

\begin{align*}
Rev &= \sum_{d_i = 1}^D \int_0^{\bar{V}} \w[d_i]{v} \phi_{d_i}(v) f_{d_i}(v) dv \\
&= \sum_{d_i = 1}^D \int_0^{\bar{V}} X'_{d_i}(v) \phi_{d_i}(v) f_{d_i}(v) dv \\
&= \sum_{d_i = 1}^D X_{d_i}\left( \bar{V} \right) \phi_{d_i}(\bar{V}) f_{d_i}(\bar{V}) - \int_0^{\bar{V}} X_{d_i}(v) \left( \phi_{d_i}(v) f_{d_i}(v) \right)' dv \\
\end{align*}

where $X_{d_i}(v) = \int_0^v \w[d_i]{z} dz$, and $\phi_{d_i}(v)$ is the standard Myerson virtual value function. Notice that $d_i X_{d_i}(v)$ is just the utility of a type $(v,d_i)$ when reporting the truth. We will focus on the regular case, i.e. $\left( \phi_{d_i}(v) f_{d_i}(v) \right)'$ is always non-negative.

\subsection{$D=2$}

For $D=2$ we're trying to solve the following:

	\[
	\begin{array}{lll}
	\textrm{max}    & \sum_{d \in \left\lbrace d_1,d_2 \right\rbrace } X_{d}\left( \bar{V} \right) \phi_{d}(\bar{V}) f_{d}(\bar{V}) - \int_0^{\bar{V}} X_{d}(v) \left( \phi_{d}(v) f_{d}(v) \right)' dv & \\
	\textrm{subject to}  &  \\
	& X''_{d}(v) \geq 0 & \forall d \in \left\lbrace d_1,d_2 \right\rbrace \\
	& 1 \geq X'_{d}(v) \geq 0 & \forall d \in \left\lbrace d_1,d_2 \right\rbrace \\
	& X_{d}(0) = 0 & \forall d \in \left\lbrace d_1,d_2 \right\rbrace \\	
	& d_1 X_{d_1}(v) \geq d_2 X_{d_2}\left( v \frac{d_1}{d_2}\right) &  \\				
	& d_2 X_{d_2}(v) \geq d_1 X_{d_1}\left( v \right) &  \\					
	\end{array}
	\]

The fourth and fifth constraints are the truthfulness constraints between $d_1$ and $d_2$ (Theorem~\ref{thm:local_to_global}). Without these constraints the solution is clear. For a fixed $X_{d_i}(\bar{V})$ the optimal thing we want to make $X_{d_i}(.)$ as small as possible, but still be able to reach $X_{d_i}(\bar{V})$ without having a slope greater than $1$. The optimal $X_{d_i}(.)$ is zero until $\bar{V} - X_{d_i} \left( \bar{V} \right)$, where it shoots up to $X_{d_i}(\bar{V})$ with a maximum slope of $1$. The last two constraints impose some extra structure the $X_{d_i}(.)$'s should satisfy.

Consider fixing some $X_{d_1}(.)$. Then, $X_{d_2}(.)$ must satisfy $$ \frac{d_1}{d_2} X_{d_1} \left( v \frac{d_2}{d_1} \right) \geq X_{d_2}(v) \geq \frac{d_1}{d_2} X_{d_1}(v).$$

\alex{figures necessary}

Then, if we fix some $X_{d_2}(\bar{V})$ (within the bounds imposed by $X_{d_1}(.)$), for the best $X_{d_2}(.)$, there exists a $v_2$, such that: (1) for all $v\geq v_2$, $X'_{d_2}(v) = 1$, and (2) for all $v<v_2$, $X_{d_2}(v) = \frac{d_1}{d_2} X_{d_1}(v)$.

Similarly, consider fixing some $X_{d_2}(.)$. We have that $$ \frac{d_2}{d_1} X_{d_2}(v)  \geq X_{d_1}(v) \geq  \frac{d_2}{d_1} X_{d_2}\left( v \frac{d_1}{d_2} \right),$$ which gives that there exists a $v_1$, such that: (1) for all $v\geq v_1$, $X'_{d_1}(v) = 1$, and (2) for all $v<v_1$, $X_{d_1}(v) = \frac{d_2}{d_1} X_{d_2}(v \frac{d_1}{d_2})$.

We have the following cases:
\begin{itemize}
\item $v_1 \leq v_2$\\
Thus, for all $v \leq v_1 \leq v_2$, $$ X_{d_1}(v) = \frac{d_2}{d_1} X_{d_2}\left( v \frac{d_1}{d_2} \right) = X_{d_1} \left( v \frac{d_1}{d_2} \right),$$ which implies that $X_{d_1}(v) = 0$, which also gives $X_{d_2}(v) = 0$. Now, for all $v \geq v_1$, we have that $X_{d_1}'(v)$, i.e. $\w[d_1]{v} = 1$; a posted price of $d_1 v_1$ for a bundle of $d_1$ items. For $v \in \left[ v_1 , v_2 \right]$, $$ X_{d_2}(v) = \frac{d_1}{d_2} X_{d_1}(v) = \frac{d_1}{d_2}(v-v_1)$$. This implies that the allocation function $\w[d_2]{v}$ is equal to $\frac{d_1}{d_2}$; for a price of $d_1 v_1$, we offer a bundle of $d_2$ items with probability $\frac{d_1}{d_2}$. For $v \geq v_2$, we have a posted price of $d_2 v_2 - (v_2 - v_1)d_1$ for a bundle of $d_2$ items. 


Notice that the same allocation rule can be induced by just two menu items (and no randomization): $d_1$ items cost $v_1 d_1$ and $d_2$ items cost $v_2 d_2 - (v_2 - v_1)d_1$.


\item $v_2 \leq v_1$ and $v_1 d_1 \leq v_2 d_2$\\
Similarly, for all $v \leq v_2$, $X_{d_2}(v) = X_{d_1}(v) = 0$, and the bundle of $d_2$ items has a posted price of $v_2 d_2$. For $v \in \left[ v_2 , v_1 \right]$, we have that $$ X_{d_1}(v) = \frac{d_2}{d_1} X_{d_2} \left( v \frac{d_1}{d_2} \right) \leq \frac{d_2}{d_1} X_{d_2} \left( v_2 \right) = 0.$$ For $v \geq v_1$, $X'_{d_1}(v) = 1$; a posted price of $d_1 v_1$ for $d_1$ items.
\item $v_2 \leq v_1$ and $v_1 d_1 > v_2 d_2$\\
%Similarly, for all $v \leq v_2$, $X_{d_2}(v) = X_{d_1}(v) = 0$, and the bundle of $d_2$ items has a posted price of $d_2 v_2$. For $v \in \left[ v_2 , \frac{d_2}{d_1} v_2 \right]$, we have $X_{d_1}(v) = \frac{d_2}{d_1} X_{d_2} \left( v \frac{d_1}{d_2} \right) = 0$. For $v \in \left[ \frac{d_2}{d_1} v_2 , v_1 \right]$, $X'_{d_1}(v) = \frac{d_1}{d_2}$, i.e. we offer a bundle of $d_1$ items with probability $\frac{d_1}{d_2}$ for a price of  $d_1 v_2$.For $v \geq v_1$, $X'_{d_1}(v) = 1$; a posted price of $d_1 v_1 - d_1 \left( v_1 \frac{d_1}{d_2} - v_2  \right)$ for $d_1$ items.
Similarly, for all $v \leq v_2$, $X_{d_2}(v) = X_{d_1}(v) = 0$, and the bundle of $d_2$ items has a posted price of $d_2 v_2$. For $v \in \left[ v_2 , \frac{d_2}{d_1} v_2 \right]$, we have $X_{d_1}(v) = \frac{d_2}{d_1} X_{d_2} \left( v \frac{d_1}{d_2} \right) = 0$. For $v \in \left[ \frac{d_2}{d_1} v_2 , v_1 \right]$, $X'_{d_1}(v) = 1$, i.e. we offer a bundle of $d_1$ items for a price of  $d_1 \frac{d_2}{d_1} v_2 = d_2 v_2$.
\end{itemize}

\subsection*{A qualitative characterization}

Succintly we have the following: let $v_1$ and $v_2$ be the values after which $(.,d_1)$ and $(.,d_2)$ type agents are allocated $d_1$ and $d_2$ items respectively. Then, the optimal auction posts a price for $d_1$ items and a price for $d_2$ items that is either: (1) $v_1 d_1$ and $v_2 d_2 - (v_2 - v_1)d_1$, (2) $v_1 d_1$ and $v_2 d_2$, or (3) $v_2 d_2$ for both. This is equivalent to the maximum of:
\begin{itemize}
\item $\max v_1 d_1 \left( 2 - F_1(v_1) - F_2(v_1) \right) + v_2 (d_2 - d_1) \left( 1 - F_2(v_2) \right)$\\
subject to $v_2 \geq v_1$.

\item $\max v_1 d_1 \left( 1 - F_1(v_1) \right) + v_2 d_2 \left( 1 - F_2(v_2) \right)$\\
subject to $v_1 \geq v_2$ and $v_1 \leq \frac{d_2}{d_1} v_2$.

\item $\max v_2 d_2 \left( 2 - F_2(v_2) - F_1(v_2 \frac{d_2}{d_1}) \right)$.

\end{itemize}

Let $\vstar{1}$ and $\vstar{2}$ be the optimal choices for $v_1$ and $v_2$. Also, let $\hat{v}_1$ and $\hat{v}_2$ be the monopoly pricing solutions, i.e. $\hat{v_i} = arg\max v d_i \left( 1 - F_i(v) \right)$. 

Then, we have the following options for $\vstar{1}$ and $\vstar{2}$: 
\begin{enumerate}
\item $\vstar{1} = \hat{v}_1$ and $\vstar{2} = \hat{v}_2$ (unconstrained version of the second bullet)
\item $\vstar{1} = arg\max v d_1 \left( 2 - F_1(v) - F_2(v) \right)$ and $\vstar{2} = \hat{v}_2$ (unconstrained version of the first bullet)
\item $\vstar{1} = \vstar{2} = arg\max v \left( d_1 (1 - F_1(v)) + d_2 (1-F_2(v)) \right)$ 
\item $\frac{d_1}{d_2} \vstar{1} = \vstar{2} = arg\max v d_2 \left( 2 - F_2(v) - F_1(v \frac{d_2}{d_1}) \right)$
\end{enumerate}

This corresponds to the following: compute $\hat{v}_1$ and $\hat{v}_2$. If $\frac{d_2}{d_1} \hat{v}_2 \geq \hat{v}_1 \geq \hat{v}_2$ we're done. Otherwise, compute $arg\max v d_1 \left( 2 - F_1(v) - F_2(v) \right)$. If it is at most $\hat{v}_2$, then pick the best option out of 2,3 and 4. If not, pick the best out of 3 and 4.


==> concave.tex <==
\section{Finding the optimal prices}

\newcommand\Item[1][]{%
  \ifx\relax#1\relax  \item \else \item[#1] \fi
  \abovedisplayskip=0pt\abovedisplayshortskip=0pt~\vspace*{-\baselineskip}}

In this section we show how to find the optimal prices for each possible number of items $d_i$, guaranteed to be the optimal auction by Theorem~\ref{thm:deterministic_auctions_are_optimal}. We do so by showing that $Rev(p_1,\dots, p_k )$ is a concave function...

\subsection*{$D = 2$}

\begin{multline*}
Rev(p_1,p_2) = p_1 d_1 \left( P_1 - F_1(p_1) + F_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - F_2(p_1) \right) \\ + p_2 d_2 \left( P_2 - F_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \right)
\end{multline*}

\paragraph{Derivatives}

\begin{itemize}
\Item
\begin{multline*}
\frac{\partial}{\partial p_1} Rev(p_1,p_2) = d_1 \left( P_1 - F_1(p_1) - p_1 f_1(p_1)  + F_2 \left( \frac{p_2d_2 - p_1d_1}{d_2 - d_1} \right) \right. \\ \left. - p_1 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - F_2(p_1) - p_1 f_2(p_1) \right) + p_2 d_2 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1})
\end{multline*}
\Item
\begin{multline*}
\frac{\partial}{\partial p_2} Rev(p_1,p_2) = d_1 p_1 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) + d_2 P_2 - p_2 d_2  f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - d_2 F_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1})
\end{multline*}

\end{itemize}

\paragraph{Second Order Partial Derivatives}

\begin{itemize}

\Item 
\begin{align*}
\frac{\partial^2}{\partial p_1} Rev(p_1,p_2) &= d_1 \left( - f_1(p_1) - f_1(p_1) - p_1 f'_1(p_1) - f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \right. \\ 
& \left.   + p_1 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - f_2(p_1) - f_2(p_1) - f'_2(p_1) \right) - p_2 d_2 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \\
&= d_1 \left( - 2 f_1(p_1) - p_1 f'_1(p_1) \right) + d_1 \left( - 2 f_2(p_1) - f'_2(p_1) \right) \\
& -2 d_1 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) + f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \left( p_1 d_1 - p_2 d_2 \right)
\end{align*}

From our assumption about $\left( \phi_i f_i \right)'$, we get that $-2 f_i(p) - f'_i(p) \leq 0$. Also, $p_1 d_1 \leq p_2 d_2$, since $d_1$ items can't cost more than $d_2$ items. Therefore, all the terms in the expression are negative; $\frac{\partial^2}{\partial p_1} Rev(p_1,p_2) \leq 0 $.

\Item 
\begin{align*}
\frac{\partial^2}{\partial p_2} Rev(p_1,p_2) &= d_1 p_1 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - d_2  f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \\ 
&- p_2 d_2 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - d_2 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \\
&= f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \left( p_1 d_1 - p_2 d_2 \right) - 2 d_2 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}),
\end{align*}

which is $\leq 0$ for similar reasons.

\Item 
\begin{align*}
\frac{\partial^2}{\partial p_1 \partial p_2} Rev(p_1,p_2) &= d_1 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) - p_1 d_1 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \\
&+ p_2 d_2 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) + d_2 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \\
&= f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \left( d_2 + d_1  \right) + f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \left( p_2 d_2 - p_1 d_1 \right)
\end{align*}

\Item 
\begin{align*}
\frac{\partial^2}{\partial p_2 \partial p_1} Rev(p_1,p_2) &= -d_1 p_1 f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) + d_1 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \\ 
&+ p_2 d_2  f'_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) + d_2 f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1})\\
&= f'_2\left( \frac{p_2d_2 - p_1d_1}{d_2 - d_1} \right) \left( p_2 d_2 - p_1 d_1 \right) + f_2(\frac{p_2d_2 - p_1d_1}{d_2 - d_1}) \left( d_1 + d_2 \right)
\end{align*}


\end{itemize}

Is
\[
\begin{bmatrix}
\frac{\partial^2}{\partial p_1} Rev(p_1,p_2) & \frac{\partial^2}{\partial p_1 \partial p_2} Rev(p_1,p_2)\\
\frac{\partial^2}{\partial p_2 \partial p_1} & \frac{\partial^2}{\partial p_2} Rev(p_1,p_2)
\end{bmatrix}
\]

negative semi-definite?




==> concave2.tex <==
\section{Finding the optimal prices}

In this section we show how to find the optimal prices for each possible number of items $d_i$, guaranteed to be the optimal auction by Theorem~\ref{thm:deterministic_auctions_are_optimal}. We do so by showing that $\rev{p_1,\dots, p_{\total}}$ is a concave function.

\subsection{Warm up: 2 prices}

Say we have prices $p_1 d_1$ and $p_2 d_2$ for $d_1$ and $d_2$ items. It must be that $p_1 d_1 \leq p_2 d_2$.  

\begin{align*}
Rev(p_1,p_2) &= p_1d_1 \left( \text{Probability that $d_1$ items are bought} \right) \\
&+ p_2d_2 \left( \text{Probability that $d_2$ items are bought} \right)
\end{align*}

Since $p_1d_1 \leq p_2d_2$, an agent with type $d_1$ never buys $d_2$ items. An agent with type $d_2$ might buy $d_1$ items, if her value is between $p_1$ and $\frac{p_2d_2-p_1d_1}{d_2- d_1}$. Now, if $p_1 > p_2$, then $p_1 > \frac{p_2d_2-p_1d_1}{d_2- d_1}$, and therefore, the probability that $d_2$ items are bought is $F_2\left( P_2 \right) - F_2\left( p_2 \right)$. The revenue in this case is $$ Rev_1( p_1,p_2 ) =  p_1d_1 \left( P_1 - F_1(p_1) \right) + p_2d_2 \left( P_2 - F_2(p_2) \right)$$.
If $p_1 \leq p_2$ then the probability that $d_2$ items are bought is $F_2\left( P_2 \right) - F_2\left( \frac{p_2d_2-p_1d_1}{d_2- d_1} \right).$ The revenue in this case is

\begin{align*}
Rev_2 \left( p_1,p_2 \right) &= p_1d_1 \left( P_1 - F_1(p_1) + F_2(\frac{p_2d_2-p_1d_1}{d_2- d_1})  - F_2(p_1) \right) \\
&\qquad + p_2d_2 \left( P_2 - F_2(\frac{p_2d_2-p_1d_1}{d_2- d_1}) \right)
\end{align*}

We will show that $\rev{p_1,p_2}$ is concave by showing that it is the minimum of two concave functions. We will show that (1) $Rev_1$ and $Rev_2$ are concave (Claim~\ref{claim:concave2}, and that (2) $\rev{p_1,p_2}$ is the minimum of $Rev_1$ and $Rev_2$ (Claim~\ref{claim:is_min}).

\begin{claim}\label{claim:is_min}
$\rev{p_1,p_2} = \min \{ Rev_1 \left( p_1,p_2 \right), Rev_2 \left( p_1,p_2 \right) \}$
\end{claim}

\begin{proof}
Consider the following two cases:
\begin{itemize}
\item $p_2 \geq p_1$. In this case, $\rev{p_1,p_2} = Rev_2(p_1,p_2)$. Consider $Rev_1 \left( p_1,p_2 \right) - Rev_2 \left( p_1,p_2 \right)$:
\begin{align*}
Rev_1 \left( p_1,p_2 \right) - Rev_2 \left( p_1,p_2 \right) &=  p_1d_1 \left( P_1 - F_1(p_1) \right) + p_2d_2 \left( P_2 - F_2(p_2) \right) \\
&\quad - p_1d_1 \left( P_1 - F_1(p_1) + F_2(\frac{p_2d_2-p_1d_1}{d_2- d_1})  - F_2(p_1) \right) \\
&\quad - p_2d_2 \left( P_2 - F_2(\frac{p_2d_2-p_1d_1}{d_2- d_1}) \right) \\
&= p_2d_2 \left( F_2(\frac{p_2d_2-p_1d_1}{d_2- d_1}) - F_2(p_2) \right) \\
&\quad + p_1d_1 \left( F_2(p_1) - F_2(\frac{p_2d_2-p_1d_1}{d_2- d_1}) \right)
\end{align*}

Since $p_2 \geq p_1$, by re-arranging we can get that $\frac{p_2d_2-p_1d_1}{d_2- d_1} \geq p_2 \geq p_1$. Moreover, we have $p_2 = \frac{d_1}{d_2}p_1 + \frac{d_2-d_1}{d_2} \frac{p_2d_2-p_1d_1}{d_2- d_1}$. We know that $(f_2 \phi_2)' \geq 0$, which implies that the revenue $R_2(p)$ from selling $d_2$ items for a price of $p$, is a concave function. Therefore:
\begin{gather*}
R_2 \left( p_2 \right) \geq \frac{d_1}{d_2}R_2 \left( p_1 \right)  + \frac{d_2-d_1}{d_2} R_2 \left( \frac{p_2d_2-p_1d_1}{d_2- d_1} \right) \\
p_2d_2 \left( 1 - F_2(p_2) \right) \geq \frac{d_1}{d_2} p_1d_2 \left( 1 - F_2(p_1) \right) + \frac{d_2-d_1}{d_2} \frac{p_2d_2-p_1d_1}{d_2- d_1} d_2 \left( 1 - F_2( \frac{p_2d_2-p_1d_1}{d_2- d_1} ) \right) \\
p_2d_2 \left( F_2( \frac{p_2d_2-p_1d_1}{d_2- d_1} ) - F_2(p_2) \right) \geq p_1d_1 \left( F_2( \frac{p_2d_2-p_1d_1}{d_2- d_1} ) - F_2(p_1) \right),
\end{gather*}
which is exactly $Rev_1 \left( p_1,p_2 \right) \geq Rev_2 \left( p_1,p_2 \right).$

Thus, we have that 
\[ \min \{ Rev_1 \left( p_1,p_2 \right), Rev_2 \left( p_1,p_2 \right) \} = Rev_2 \left( p_1,p_2 \right) = \rev{p_1,p_2}. \]
\item $p_2 \leq p_1$. In this case, $\rev{p_1,p_2} = Rev_1(p_1,p_2)$. Using a similar proof, we can show that $Rev_1 \left( p_1,p_2 \right) - Rev_2 \left( p_1,p_2 \right) \leq 0$.

\end{itemize}

\end{proof}



==> d_2.tex <==
\subsection{$\total=2$}\label{subsec:d=2}
%For a fixed $U_{d_i}(\bar{V})$ and $U_{d_j}(.)$ we want to make $U_{d_i}(.)$ as small as possible, but still be able to reach $U_{d_i}(\bar{V})$ without having a slope greater than $1$, and still be within the bounds imposed by $U_{d_j}$.

%The optimal $U_{d_i}(.)$ is zero until $\bar{V} - U_{d_i} \left( \bar{V} \right)$, where it shoots up to $U_{d_i}(\bar{V})$ with a maximum slope of $1$. The last two constraints impose some extra structure the $U_{d_i}(.)$'s should satisfy.

%Suppose we fix some $U_{d_1}(.)$. Then, $U_{d_2}(.)$ must satisfy $$ \frac{d_1}{d_2} U_{d_1} \left( v \frac{d_2}{d_1} \right) \geq U_{d_2}(v) \geq \frac{d_1}{d_2} U_{d_1}(v).$$
%Further, fix some $U_{d_2}(\bar{V})$ (within the bounds imposed by $U_{d_1}(.)$). 
%Since $\left( \phi_{d}(v) f_{d}(v) \right)'$ is non-negative, we could try to minimize $U_{d_2}(.)$ pointwise, but this might result in violating the lower bound imposed by $U_{d_1}(.)$. The point-wise minimum
Fix some function $U_{d_1}(.)$ and a value $U_{d_2}(\bar{V})$. Given these, the optimum $U_{d_2}(.)$ is going to be the pointwise minimum function that satisfies all the constraints of the mathematical program  (\ref{eq:mathprog}). Lemma~\ref{lem:shootinup} describes exactly the structure of $U_{d_2}(.)$: in some interval $[0,v'_2]$ we have $U_{d_2}(v) = 0$ (case 4 of the Lemma). In some interval $[v'_2,v_2]$ we have $U_{d_2}(v) = \frac{d_1}{d_2} U_{d_1}(v)$ (case 3), and in the interval $[v_2,\bar{V}]$ we have $U'_{d_2}(v) = 1$ (case 1). This description can be simplified to: there exists a $v_2$, such that: (1) for all $v\geq v_2$, $U'_{d_2}(v) = 1$, and (2) for all $v<v_2$, $U_{d_2}(v) = \frac{d_1}{d_2} U_{d_1}(v)$. See Figure~\ref{fig:Xd2} for a depiction of this.

%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}[hbt]
\centering
\begin{tikzpicture}[scale=1]
%  \draw[style=help lines] (0,0) grid (3.9,3.9);

  \draw[->] (-0.2,0) -- (4.3,0) node[right] {$v$};
  \draw[->] (0,-0.2) -- (0,4);

  \draw (0,0) parabola bend (0,0) (4,4) node[above left] {$U_{d_1}(.)$};
  \draw (0,0) parabola bend (0,0) (4,2) node[below right] {$\frac{d_1}{d_2} U_{d_1}(.)$};
  \draw[red] (2,0.5) -- (4,3) node[below right] {$U_{d_2}(.)$};
  \draw[red] (0,0) parabola bend (0,0)(2,0.5);
  \draw[dashed] (2,0.5) -- (2,0) node[below] {$v_2$};
  \filldraw (4,0) circle (1pt) node[below] {$\bar{V}$};
\end{tikzpicture}
\caption{Pointwise minimum $U_{d_2}(.)$, given $U_{d_1}$ and $U_{d_2}(\bar{V})$}
\label{fig:Xd2}
\end{figure}
%\end{wrapfigure}
%Notice that $U_{d_2}(v) = \frac{d_1}{d_2} U_{d_1}(v)$ implies that the utility of a type $(v,d_2)$ when reporting the truth is equal to her utility when reporting $(v,d_1)$.

Similarly, fixing $U_{d_2}(.)$, gives that there exists a $v_1$, such that: (1) for all $v\geq v_1$, $U'_{d_1}(v) = 1$, and (2) for all $v<v_1$, $U_{d_1}(v) = \frac{d_2}{d_1} U_{d_2}(v \frac{d_1}{d_2})$. 

Now consider the menu representation of a mechanism that induces utility functions $U_{d_1}(.)$ and $U_{d_2}(.)$.  By the above analysis, such a mechanism offers, among other lotteries, deterministic allocations of $d_1$ and $d_2$ items.  More specifically, for $v \geq v_1$ we have $U'_{d_1}(v)=1$, and the allocation of type $(v,d_1)$ is $w_{d_1}(v) = U'_{d_1}(v) = 1$ (and similarly for a type $(v,d_2)$).  In particular, types $(\bar{V},d_1)$ and $(\bar{V},d_2)$ choose deterministic allocations of $d_1$ and $d_2$ items, respectively.   Now construct an alternative mechanism that removes all choices other than the deterministic allocations from the menu.  The alternative menu contains two options, namely deterministic allocations of $d_1$ and $d_2$ items (for the same prices as the original mechanism).  Note that the utility function of the alternative mechanism is pointwise weakly lower than the utility function of the original mechanism, since each type faces a smaller menu of choices.  Furthermore, the utility of types $(\bar{V},d_1)$ and $(\bar{V},d_2)$ remains the same, since the deterministic allocations that they chose in the original mechanism are still available in the alternative mechanism.  By price-regularity, the revenue of the alternative mechanism is no lower than the revenue of the original mechanism.  A more detailed case analysis is provided in Appendix~\ref{app:detailed d2}.  Using this characterization we show how to find these critical values in the appendix. 


==> deterministic.tex <==
\section{Deterministic}

If the auction is deterministic, then we have that:
\[ u_{(v_i,d_i)}(v_j,d_j) = v_i \min\left( d_i , x(v_j,d_j) \right) - p(v_j,d_j) \]

\begin{claim}
If $x(t_i) = x(t_j) = k$ then $p(t_i) = p(t_j) = p_k$, and vice versa, i.e. a truthful mechanism has a price per bundle of items.
\end{claim}

It is also easy to see that $p_k$ is increasing in $k$.

\begin{conjecture}
The deterministic revenue maximizing auction is NP-hard to compute.
\end{conjecture}

==> general_d.tex <==
\subsection{General $\total$}\label{subsec:general_d}
%\nikhil{Add why we need monotone paths, aka Lemma \ref{lem:monotone paths}.} 
For a given type, Corollary \ref{cor:derivatives_left_and_right} may only give us relative proportions of the allocation probability. 
We can combine a sequence of these tight constraints until we get to a type whose allocation probability is either 0 or 1. 
This would then give us the allocation probability to be some rational number, but not necessarily of the form 
$\frac {d'}d$.
For instance, it could be that 
$$U'_{d_i}(v)  = \frac{d_{i-1}}{d_i} U'_{d_{i-1}} (v) = \frac{d_{i-1}}{d_i}U'_{d_i}(\frac{d_{i-1}}{d_i} v) 
=   \frac{d_{i-1}^2}{d_i^2} U'_{d_{i-1}}(\frac{d_{i-1}}{d_i} v)  = \frac{d_{i-1}^2}{d_i^2}.$$
Fortunately, we can rule out such sequence of tight constraints.
We can show that the sequence of tight constraints must be such that  the $d_i$s cancel out 
and we get the allocation probability to be of the form $\frac {d'} d $ as required. 


%We now further exploit the structure of the equalities implied by Lemma~\ref{lem:shootinup}.  
%The key facts that we use from what we have proved so far are  that 
% for a type with a probabilistic allocation, her utility  when reporting her true type is equal to her utility when reporting some other type, and that the allocation probabilities are propoertional . 
%\begin{lemma}\label{lem:shoot_up}
%There exist values $v_1, \dots, v_k$ such that all types $(v,d_i)$, with $v \geq v_i$ buys $d_i$ items.
%\end{lemma}
%
%\begin{lemma}\label{lem:shoot_up_2}
%	In the optimal solution, for each type $(v,d_i)$ that buys $d_i$ items with probability less than one, there exists another type $(v',d')$ such that $(v,d_i)$ gets the same utility from the allocation of $(v',d')$.
%\end{lemma}
%\begin{proof}
%Assume this is not the case. Recall that maximizing revenue for fixed $U_{d_i}(\hat{V})$ and fixed $U_{d}(.)$, for all $d \neq d_i$ is equivalent to point wise minimizing $U_{d_i}(.)$. If after point wise minimizing there exists a type $(v,d_i)$ that buys $d_i$ items with probability less than one, it must be that one or more of the IC constraints associated with this type are tight. From Theorem~\ref{thm:local_to_global} we know that $\ut{v,d_i}{v, d_i} = d_i U_{d_i}(v)$ is bounded from bellow from $\ut{v,d_i}{v \frac{d_i}{d_j}, d_j} = d_j U_{d_j}(v\frac{d_i}{d_j})$, for all $d_j > d_i$, and $\ut{v,d_i}{v , d_k} = d_k U_{d_k}(v)$, for all $d_k < d_i$. One of these constraints must be tight; the Lemma follows.
%\end{proof}


	Consider a graph with a node for each type.  For each type $(v,d_i)$ such that $1> U'_{d_i}(v)>0$, 
	add a directed edge to either $\left(v\frac{d_i}{d_{i+1}} , d_{i+1} \right)$ or 
	$(v,d_{i-1})$, if the corresponding constraints from  Lemma~\ref{lem:shootinup}  is tight. 
From Lemma~\ref{lem:utilandX}, whenever there is an edge from $(v,d)$ to $(v',d')$, then the buyer with type $(v,d)$ gets the same utility from the allocation of $(v',d')$.  
We claim that this graph is acyclic. 
This follows from the observation that if you start from $(v,d)$ and a sequence of edges brings you to $(v',d)$, then $v'$ 
must be strictly smaller that $v$. Going left does not change $v$ whereas going right strictly decreases it.
In fact, the crucial structure of this graph that we use is that a path can either go only left, or only right, unless the utilities are all 0, as stated in the following lemma.  
\begin{restatable}{lemma}{monotonePaths}\label{lem:monotone paths}
%A directed path starting from $(v,d_i)$, such that $d_i U_{d_i}(v) > 0$, is either monotone increasing or monotone decreasing in $d$.
If the directed path starting from $(v,d_i)$ is non-monotone in $d_i$, then $d_i U_{d_i}(v) = 0$.
\end{restatable}
\begin{proof}
	There are two cases: either the edge exiting $(v,d_i)$ is to $(v,d_{i-1})$ or $\left(v\frac{d_i}{d_{i+1}} , d_{i+1} \right)$.  
	
	In the first case, let $(v,d_j)$ be the first vertex such that there is an edge from $(v,d_j)$ to $(v\frac{d_j}{d_{j+1}} , d_{j+1})$. Also, since $(v,d_j)$ is the first such vertex, there must be an edge from $(v,d_{j+1})$ to $(v,d_j)$. The existence of these edge gives $d_{j+1} U_{d_{j+1}} \left( v \right) = d_j U_{d_j}(v) = d_{j+1} U_{d_{j+1}} \left( v \frac{d_j}{d_{j+1}} \right)$. From Lemma \ref{lem:shootinup}, the only way this is  possible is if $U_{d_{j+1}}(.)$ is zero in the range $[ v \frac{d_j}{d_{j+1}} , v ]$, which implies that $d_i U_{d_i}(v) = 0$. The latter case is identical.
\end{proof}


%Combining the structure of the path starting from $(v,d_i)$ and \Cref{lem:utilandX} we get:

%\begin{corollary}\label{cor:same utility on path}
%$(v,d)$ has the same utility from the allocation of $(v,d')$, for all $(v,d')$ on the path that starts from $(v,d)$.
%\end{corollary}

We are now ready to prove our claim from the beginning of this section, that the allocation probabilities must be equal to ratios of demands, which immediately implies \autoref{thm:deterministic}.

\begin{lemma}\label{lem:exists paths to deterministic alloc}
	In a solution to (\ref{eq:mathprog}) that satisfies Lemma~\ref{lem:shootinup}, for each type $(v,d)$, 
	the allocation probability  $U'_{d}(v)$ is either 0, 1, or $d'/d$ for some smaller demand $d'$. 
	%strictly between 0 and 1, there exists another type $(v,d')$ such that 
	%$U'_{d'}(v) =1$, and $(v,d)$ gets the same utility of $dU_d(v)$  from the allocation of $(v,d')$ and the same payment as $(v,d')$.
\end{lemma}
\begin{proof}

	Consider any type $(v,d)$ such that $U'(v,d)$ is strictly between 0 and 1. From Lemma~\ref{lem:shootinup}, there must be an outgoing edge from this node. Consider an arbitrary path that starts with $(v,d)$ and ends in a vertex $(v',d')$ with no outgoing edges. By Lemma~\ref{lem:shootinup}, $(v',d')$ must get $d'$ items with probability one, otherwise $(v',d')$ will have an outgoing edge.	By Lemma~\ref{lem:monotone paths}, the path is either increasing or decreasing in $d$. If it is increasing in $d$, then by Corollary~\ref{cor:derivatives_left_and_right}, $U'_d(v) = U'_{d'}(v') = 1$. If it is decreasing in $d$, then $v'=v$, and by Corollary~\ref{cor:derivatives_left_and_right} and a telescoping product we have $U'_d(v) = \frac{d'}{d} U'_{d'} (v')= \frac{d'}{d}$.
\end{proof}

\begin{proof}[Proof of \autoref{thm:deterministic}]
	Consider a mechanism that satisfies conditions of Lemma \ref{lem:shootinup}.  
	By Lemma \ref{lem:exists paths to deterministic alloc}, if type $t = (v,d)$ has a probabilistic allocation, then that allocation is of the form $\frac{d'}{d}$, for some $d' < d$. Therefore, we can keep her payment the same, and 
replace her allocation with a deterministic allocation of $d'$ items. The new mechanism has the same revenue and is deterministic. The initial mechanism was arbitrary. Therefore, for every solution to (\ref{eq:mathprog}), there exists a deterministic solution with revenue at least as large, and therefore the optimal solution to (\ref{eq:mathprog}) exists and is deterministic.
\end{proof}
